UCE-FID: Using Large Unlabeled, Medium Crowdsourced-Labeled, and Small Expert-Labeled Tweets for Foodborne Illness Detection

Foodborne illnesses significantly impact public health. Deep learning surveillance applications using social media data aim to detect early warning signals. However, labeling foodborne illness-related tweets for model training requires extensive human resources, making it challenging to collect a sufficient number of high-quality labels for tweets within a limited budget. The severe class imbalance resulting from the scarcity of foodborne illness-related tweets among the vast volume of social media further exacerbates the problem. Classifiers trained on a class-imbalanced dataset are biased towards the majority class, making accurate detection difficult. To overcome these challenges, we propose EGAL, a deep learning framework for foodborne illness detection that uses small expert-labeled tweets augmented by crowdsourced-labeled and massive unlabeled data. Specifically, by leveraging tweets labeled by experts as a reward set, EGAL learns to assign a weight of zero to incorrectly labeled tweets to mitigate their negative influence. Other tweets receive proportionate weights to counter-balance the unbalanced class distribution. Extensive experiments on real-world \textit{TWEET-FID} data show that EGAL outperforms strong baseline models across different settings, including varying expert-labeled set sizes and class imbalance ratios. A case study on a multistate outbreak of Salmonella Typhimurium infection linked to packaged salad greens demonstrates how the trained model captures relevant tweets offering valuable outbreak insights. EGAL, funded by the U.S. Department of Agriculture (USDA), has the potential to be deployed for real-time analysis of tweet streaming, contributing to foodborne illness outbreak surveillance efforts.

==> section/old_sec_4_experiments.tex <==
\section{experiments}

\subsection{Experiment Settings}

\subsubsection{Text Relevance Classification (TRC) Task} This task, introduced by \cite{hu2022tweet}, aims to identify tweets that refer to a foodborne illness incident. Each tweet in Tweet-FID has a binary label indicating its relevance to foodborne illness. This task can help detect potential outbreaks of foodborne diseases from social media posts.


\subsubsection{Dataset} 
We use Tweet-FID, the publically available
dataset from \cite{hu2022tweet}, which contains 1,362 (33$\%$) relevant and 2,760(67$\%$) irrelevant tweets for the TRC task. Each tweet has an expert label and an aggregated crowdsourced label. The dataset was split based on expert labels, the training set consists of 1,088 relevant tweets and 2,210 irrelevant tweets. The validation set includes 137 relevant tweets and 275 irrelevant tweets. The test set consists of 137 relevant tweets and 275 irrelevant tweets.  Aggregated crowdsourced labels regard 1,625 tweets as relevant and 1,673 tweets as irrelevant. The noise ratio, defined as the ratio of the difference between aggregated crowdsourced labels and expert labels to the total number of labels  in the training dataset, is 20.29\%.  It is important to note that we only utilize expert labels for the validation and test sets. In our experiments, we combine the validation and test sets to create a new validation set, which is used exclusively for validation purposes. The expert-labeled reward set for meta-learning-based methods is not a subset of this new validation set; instead, the instances in the expert-labeled reward set are derived from the training set.
Additionally, we now also utilize the unlabeled tweets collected with the same domain-specific keywords as in \cite{hu2022tweet}. We filter out tweets with less than 5 tokens since they are typically not sufficiently informative. In the end, we are left with 50,000 tweets as an unlabeled set used in our experiment.


\subsubsection{Baseline Methods}


For a fair comparison, we adopt a pre-trained RoBERTa \cite{liu2019roberta} as the backbone model for all compared methods. RoBERTa is an improved version of BERT \cite{devlin2018bert} that removes the next-sentence prediction task and uses larger learning rates and mini-batches for pre-training. RoBERTa has achieved state-of-the-art performance on multiple tasks \cite{liu2019roberta}, including the TRC task \cite{hu2022tweet}. We compare \modelabbr{} with following methods:

{\bf Fully supervised learning. (Sup. Learning)} 
Sup. Learning trains a text classification model on the given labeled data without any special treatment for addressing label noise. This method also does not use any unlabeled data.

{\bf SoftMatch.} 
Softmatch, proposed by \cite{chen2023softmatch}, is a state-of-the-art semi-supervised learning method for balanced and imbalanced classification. It balances the quality and quantity of pseudo-labels by using a truncated Gaussian function based on sample confidence. Softmatch also encourages diverse pseudo-labels using a uniform alignment approach. It has achieved significant improvements, particularly in tasks with imbalanced class distributions.

{\bf CWSL.}
This is a weakly-supervised learning method proposed by \cite{Guo_Kuang_Liu_Li_Ma_Qie_2020}. It is designed to cope with severe label noise by assigning small weights to noisy instances. The instance reweight process is under the guidance of performance on a clean reward dataset. CWSL adopts robust AUC criteria as performance measurement on the reward set to conquer the issue that the label distributions in the training and testing data are different.

{\bf COSINE.}
This  self-training approach \cite{yu2021fine}  fine-tunes a pre-trained language model using both weakly labeled and unlabeled data.  COSINE first fine-tunes the pre-trained model with the weakly-labeled data and then generates pseudo-labels for the unlabeled data. COSINE applies contrastive regularization and confidence-based sample reweighting to enhance model performance and mitigate error propagation during the self-training procedure.

\input{table/setting}
\subsubsection{Experimental Setting}
All experiments are conducted on a server with an A100-80G GPU. All code is developed with Python 3.9 on PyTorch 1.12.0.

{\bf Methodology.} For our tweet-fid dataset, we treat expert labels as ground-truth labels and consider crowdsourced labels as noisy labels. We vary the expert label ratio in the labeled training set (LTS) among 0\%, 10\%, 20\%, and 30\% to analyze the performance of each method in a wide variety of scenarios. For semi-supervised methods, we use the 50,000 unlabeled tweets that we collected as an unlabeled training set (UTS) to train these methods. We consider two scenarios for methods that learn weights from an expert-labeled reward set (ELRS): (1) ELRS consists of all the expert-labeled tweets in the LTS. (2) All tweets in LTS are with their \textbf{crowdsourced labels}, and we randomly sample $k\%$ of tweets from LTS to create an ELRS with their \textbf{expert labels}. $k$ ranges in $[10\%, 20\%, 30\%]$. In both scenarios, the ELRS tweets are also in LTS. All experimental settings are shown in Table \ref{tab: setting}. For those experimental settings involving expert labels, we create 5 datasets. In each dataset, expert labels were assigned to different tweets.

In our experiment, we utilize the Adam optimizer \cite{kingma2014adam} with a learning rate of $1 \times 10^{-5}$, $\beta_{1}$ of 0.9, $\beta_{2}$ of 0.999, weight decay of $1 \times 10^{-4}$, and layer decay of 0.75 to train each neural network model. For \modelabbr{}, we set the $\beta$ value in Eq. (\ref{eq:lt}) to 1. Each model is trained for a total of 10,000 steps. Throughout the training process, we utilize a separate expert-labeled validation dataset (not the reward set) to evaluate the model's performance every 512 steps. The model's best performance is recorded based on the metrics described in the subsequent subsubsection.



% In our experiment, we have three types of data: expert-labeled tweets, crowdsource-labeled tweets, and unlabeled tweets. However, some methods cannot utilize all three types of data. We created 10 types of data settings and assign each method with appropriate settings that can handle with. Each setting is introduced below:

% {\bf Setting 1: Expert-labeled training set only.} In this setting, all labels in the training set are expert labels, which means there are no noisy labels in the training set. Unlabeled tweets are not used during the training procedure.

% {\bf Setting 2: Crowdsource-labeled training set only.} In this setting, all labels in the training set are crowdsourced labels, which means there are some inaccurate labels in the training set. Unlabeled tweets are not used during the training procedure.

% {\bf Setting 3: Mix-labeled training set only.} In this setting, we randomly select a small proportion of tweets in training data and assign selected tweets with expert labels, the other tweets in the training dataset are with crowdsourced labels. Unlabeled tweets are not used during the training procedure.

% {\bf Setting 4: Crowdsource-labeled training set + small expert-labeled validation set.} This setting uses only crowdsourced labels for the training set, but also has a small validation set with expert labels. The validation set helps to adjust the weights of the training instances based on their quality. The validation set is a subset of the training set. No unlabeled tweets are used in this setting.

% {\bf Setting 5: Mix-labeled training set + small expert-labeled validation set.} This setting uses a mix of crowdsourced and expert labels for the training set, where a small fraction of tweets are randomly selected and labeled by experts. These expert-labeled tweets also form the validation set. No unlabeled tweets are used in this setting.

% {\bf Setting 6: Expert-labeled and unlabeled training set.} This setting uses both labeled and unlabeled tweets for the training set, where all the labeled tweets have expert labels. This setting leverages the unlabeled data to augment the training set.

% {\bf Setting 7: Crowdsource-labeled and unlabeled training set.} This setting uses only crowdsourced labels for the labeled tweets in the training set, and also includes unlabeled tweets. This setting exploits the unlabeled data to supplement the training set.

% {\bf Setting 8: Mix-labeled and unlabeled training set.} This setting uses a combination of crowdsourced and expert labels for the labeled tweets in the training set, where a small fraction of tweets are randomly selected and labeled by experts. This setting also uses unlabeled tweets to augment the training set.

% {\bf Setting 9: Crowdsource-labeled and unlabeled training set + small expert-labeled validation set.} This setting uses only crowdsourced labels for the labeled tweets in the training set, and also includes unlabeled tweets. Additionally, this setting has a small validation set with expert labels, which is a subset of crowdsource-labeled tweets training set. The validation set helps to adjust the weights of the training instances based on their quality.

% {\bf Setting 10: Mix-labeled and unlabeled training set + small expert-labeled validation set.} This setting uses a mix of crowdsourced and expert labels for the labeled tweets in the training set, where a small fraction of tweets are randomly selected and labeled by experts. These expert-labeled tweets also form the validation set. This setting also uses unlabeled tweets to supplement the training set.

% Each method is assigned with settings described above.


\subsubsection{Evaluation Metrics}
We use standard accuracy, F1, and balanced accuracy (bACC) \cite{huang2016learning, wang2017learning} to measure each method's performance. These three metrics can illustrate a method's performance from various perspectives given an imbalanced class distribution.

\subsection{Performance}
\input{table/performance_mix}
\input{table/performance_crowdonly}

Table \ref{tab:mix} provides a comparison of different methods' performance when the training data includes both expert labels and crowdsourced labels. It is evident that SoftMatch, a semi-supervised method that incorporates unlabeled data, outperforms the supervised learning method that relies solely on labeled data. However, COSINE, another method designed for learning with weakly-labeled and unlabeled data, does not demonstrate any advantage over the supervised method, likely due to its limitations in handling imbalanced classification problems and lack of guidance from expert-labeled data. Methods utilizing a small reward set with expert labels show superior performance compared to the supervised learning method. Notably, our method \modelabbr{} achieves the most promising results by effectively leveraging both unlabeled data and the reward set. This indicates that \modelabbr{} successfully utilizes the reward set to assign appropriate weights to training tweets, mitigating the impact of noisy labels and addressing the class imbalance problem.

In Table \ref{tab:crowdonly}, we present the results obtained when the training data lacks expert labels. It is important to note that all methods perform worse compared to their counterparts in Table \ref{tab:mix}, highlighting the negative influence of label noise. However, even in this scenario, SoftMatch outperforms the supervised method. Additionally, methods that leverage the small expert-labeled reward set demonstrate superior performance compared to the supervised learning method. Once again, our method \modelabbr{} maintains its position as the top-performing approach among all methods.



\subsection{Case Study}
% In 2021, the Centers for Disease Control and Prevention (CDC) and the Food and Drug Administration (FDA) conducted an investigation into a multistate outbreak of Salmonella Typhimurium infections \cite{CDC2021}. The investigation revealed that BrightFarms brand packaged salad greens were responsible for causing illnesses in individuals across four states. A total of 31 cases of infection with the outbreak strain of Salmonella Typhimurium were officially reported. However, it is highly likely that the actual number of affected individuals in this outbreak exceeds the reported cases, and the outbreak may extend beyond the states with confirmed illnesses. This is primarily due to the fact that many people recover from the illness without seeking medical care and therefore do not undergo testing for \textit{Salmonella} \cite{CDC2021}. 

% In this study, we utilized our proposed method, \modelabbr{}, to identify tweets that could potentially be related to the specific outbreak under investigation. Following the data collection approach outlined in \cite{hu2022tweet}, we gathered tweets with geotags from the year 2021. We filtered out tweets originating from locations outside the United States. Subsequently, we employed our trained \modelabbr{} model to predict whether these tweets mentioned cases of foodborne illness. We retained the tweets that were predicted to be relevant to foodborne illness and contained keywords such as "salad" and "greens".
In 2021, the CDC and FDA investigated a Salmonella Typhimurium outbreak \cite{CDC2021}, linking it to BrightFarms brand packaged salad greens in four states. Officially, 31 cases were reported, but the actual number is likely higher due to underreporting and mild cases not seeking medical care \cite{CDC2021}. Using our method, \modelabbr{}, we identified tweets potentially related to this outbreak. Following the approach in \cite{hu2022tweet}, we collected geotagged tweets from 2021, filtering out non-U.S. locations. Our trained \modelabbr{} model predicted relevant foodborne illness tweets mentioning keywords like "salad" and "greens".

\input{fig/tweet_cdc}

Figure \ref{fig:tweet_cdc} presents the weekly count of relevant tweets throughout 2021 (represented by the light blue curve) and its corresponding moving average (displayed as the yellow curve, with a sampling width of 4). The figure also includes the weekly number of reported cases recorded by the CDC \footnotemark[\value{footnote}] (indicated by the red curve). Notably, during the period from May to August 2021, there was a noticeable increase in the number of tweets referencing foodborne illness and containing the specified keywords. The reported cases of illness commenced between June 10, 2021, and August 18, 2021. However, it is important to acknowledge that the actual outbreak might have started prior to the first reported case and could have persisted beyond the detection of the last reported case. The tweets captured by \modelabbr{} offer insights into the trend of this outbreak. This highlights the potential of our method, \modelabbr{}, in detecting early signals of possible foodborne illness outbreaks.

==> table/performance_crowdonly_30.tex <==

\begin{table}[htb]
\caption{Performance comparison of all methods when expert labels are not in the labeled training dataset. 
}
    \centering
    \begin{tabular}{cccc}
    \hline
        Method & F1 & Accuracy & bACC \\ \hline
        Sup. Learning & 0.789 ± 0.007 & 0.828 ± 0.009 & 0.862 ± 0.005 \\ 
        Softmatch* & 0.797 ± 0.004 & 0.837 ± 0.003 & 0.862 ± 0.006 \\ 
        COSINE* & 0.767 ± 0.011	& 0.811 ± 0.014 & 0.843 ± 0.008 \\ 
        CWSL\textsuperscript{$\#$} & 0.808 ± 0.008 & 0.850 ± 0.009 & 0.875 ± 0.005 \\ 
        EGAL*\textsuperscript{$\#$} & \textbf{} & \textbf{} & \textbf{} \\ \hline
    \end{tabular}
\label{tab: crowd30}

\end{table}

% \begin{table}[!t]
% \caption{Performance of methods trained on crowdsourced labeled set $D^c$ and $\Tilde{D}^c$. *: the method utilizes the unlabeled training set. \textsuperscript{$\#$}: the method utilizes expert-labeled reward set.}
% \label{tab:crowdonly_mix}

%     \begingroup
%     \setlength{\tabcolsep}{5.5pt} % Default value: 6pt
%     \renewcommand{\arraystretch}{1.25} % Default value: 1
%     \begin{tabular}{lcccc}
%     \hline
%         ~ & Method & F1 & Accuracy & bACC \\ \hline
% \multirow{4}{*}{$D^c$} & Sup. Learning & 0.789 ± 0.007 & 0.828 ± 0.009 & 0.862 ± 0.005 \\ 
%          & Softmatch* & 0.797 ± 0.004 & 0.837 ± 0.003 & 0.862 ± 0.006 \\ 
%         & COSINE* & 0.733 ± 0.014 & 0.767 ± 0.017 & 0.816 ± 0.013 \\ 
%         & CWSL\textsuperscript{$\#$} & 0.808 ± 0.008 & 0.850 ± 0.009 & 0.875 ± 0.005 \\ 
%         & EGAL*\textsuperscript{$\#$} & \textbf{0.820 ± 0.004} & \textbf{0.868 ± 0.004} & \textbf{0.877 ± 0.004} \\ \hline
% \multirow{4}{*}{$\Tilde{D}^c$} & Sup. Learning & 0.798 ± 0.009 & 0.848 ± 0.004 & 0.871 ± 0.003 \\ 
%         & Softmatch* & 0.807 ± 0.005 & 0.850 ± 0.007 & 0.873 ± 0.002 \\ 
%         & COSINE* & 0.755 ± 0.010 & 0.803 ± 0.003 & 0.833 ± 0.007 \\ 
%         & CWSL\textsuperscript{$\#$} & 0.812 ± 0.009 & 0.856 ± 0.009 & 0.876 ± 0.007 \\ 
%         & EGAL*\textsuperscript{$\#$} &  \textbf{0.826 ± 0.008} & \textbf{0.870 ± 0.008} & \textbf{0.885 ± 0.006} \\ \hline
%     \end{tabular}
%     \endgroup
% \end{table}

==> table/performance_mix_30.tex <==
\begin{table}[htb]
\caption{Performance comparison of all methods when expert labels are not in the labeled training dataset. *: the method utilizes the unlabeled training set. \textsuperscript{$\#$}: the method utilizes expert-labeled reward set.}
    \centering
    \begin{tabular}{cccc}
    \hline
        Method & F1 & Accuracy & bACC \\ \hline 
        Sup. Learning & 0.798 ± 0.009 & 0.848 ± 0.004 & 0.871 ± 0.003 \\ 
        Softmatch* & 0.807 ± 0.005 & 0.850 ± 0.007 & 0.873 ± 0.002 \\ 
        COSINE* & 0.785 ± 0.002	& 0.835 ± 0.002	& 0.854 ± 0.003 \\ 
        CWSL\textsuperscript{$\#$} & 0.812 ± 0.009 & 0.856 ± 0.009 & 0.876 ± 0.007 \\ 
        EGAL*\textsuperscript{$\#$} &  \textbf{0.823 ± 0.012} & \textbf{0.867 ± 0.011} & \textbf{0.883 ± 0.009} \\ \hline
    \end{tabular}
\label{tab: mix30}		

\end{table}
